Understanding how people consume low quality and extreme news using web traffic data

To mitigate the spread of fake news, researchers need to understand who visit fake new sites, what brings people to those sites, where visitors come from, and what content they prefer to consume. In this paper, we analyze web traffic data from The Gateway Pundit (TGP), a popular far-right website that is known for repeatedly sharing false information that has made its web traffic available to the general public. We collect data on 68 million web traffic visits to the site over a month period and analyze how people consume news via multiple features. Our traffic analysis shows that search engines and social media platforms are main drivers of traffic; our geo-location analysis reveals that TGP is more popular in counties that voted for Trump in 2020; and our topic analysis shows that conspiratorial articles receive more visits than factual articles. Due to the inability to observe direct website traffic, existing research uses alternative data source such as engagement signals from social media posts. To validate if social media engagement signals correlate with actual web visit counts, we collect all Facebook and Twitter posts with URLs from TGP during the same time period. We show that all engagement signals positively correlate with web visit counts, but with varying correlation strengths. Metrics based on Facebook posts correlate better than metrics based on Twitter. Our unique web traffic data set and insights can help researchers to better measure the impact of far-right and fake news URLs on social media platforms.

==> OLD_bib_with_url_entry.tex <==

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

@article{COVID-19-infodemic,
	Author = {Cinelli, Matteo and Quattrociocchi, Walter and Galeazzi, Alessandro and Valensise, Carlo Michele and Brugnoli, Emanuele and Schmidt, Ana Lucia and Zola, Paola and Zollo, Fabiana and Scala, Antonio},
	Da = {2020/10/06},
	Date-Added = {2021-01-07 17:25:26 +0000},
	Date-Modified = {2021-01-07 17:25:26 +0000},
	Doi = {10.1038/s41598-020-73510-5},
	Id = {Cinelli2020},
	Isbn = {2045-2322},
	Journal = {Scientific Reports},
	Number = {1},
	Pages = {16598},
	Title = {The COVID-19 social media infodemic},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/s41598-020-73510-5},
	Volume = {10},
	Year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1038/s41598-020-73510-5},
	Bdsk-Url-2 = {http://dx.doi.org/10.1038/s41598-020-73510-5}
}
@article{Hoaxy,
   title={Hoaxy},
   ISBN={9781450341448},
   url={http://dx.doi.org/10.1145/2872518.2890098},
   DOI={10.1145/2872518.2890098},
   journal={Proceedings of the 25th International Conference Companion on World Wide Web - WWW  ’16 Companion},
   publisher={ACM Press},
   author={Shao, Chengcheng and Ciampaglia, Giovanni Luca and Flammini, Alessandro and Menczer, Filippo},
   year={2016}
}
@article{FakeNewsTracker,
	Author = {Shu, Kai and Mahudeswaran, Deepak and Liu, Huan},
	Da = {2019/03/01},
	Date-Added = {2021-01-07 17:21:29 +0000},
	Date-Modified = {2021-01-07 17:21:29 +0000},
	Doi = {10.1007/s10588-018-09280-3},
	Id = {Shu2019},
	Isbn = {1572-9346},
	Journal = {Computational and Mathematical Organization Theory},
	Number = {1},
	Pages = {60--71},
	Title = {FakeNewsTracker: a tool for fake news collection, detection, and visualization},
	Ty = {JOUR},
	Url = {https://doi.org/10.1007/s10588-018-09280-3},
	Volume = {25},
	Year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1007/s10588-018-09280-3},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/s10588-018-09280-3}
}
@inproceedings{factoring-fact-checks,
author = {Jiang, Shan and Baumgartner, Simon and Ittycheriah, Abe and Yu, Cong},
title = {Factoring Fact-Checks: Structured Information Extraction from Fact-Checking Articles},
year = {2020},
isbn = {9781450370233},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3366423.3380231},
doi = {10.1145/3366423.3380231},
booktitle = {Proceedings of The Web Conference 2020},
pages = {1592–1603},
numpages = {12},
keywords = {information extraction, misinformation, sequence tagging, BERT, ClaimReview, computational journalism, fact-checking},
location = {Taipei, Taiwan},
series = {WWW '20}
}
@manual{traffic-manipulation-on-twitter,
      title  = {Measuring traffic manipulation on Twitter},
      author = {Ben Nimmo},
      url    = {https://comprop.oii.ox.ac.uk/wp-content/uploads/sites/93/2019/01/Manipulating-Twitter-Traffic.pdf},
      year   = {2021 (accessed January 5, 2021}
}
@manual{breakout-scale,
      title  = {THE BREAKOUT SCALE:
MEASURING THE IMPACT OF INFLUENCE OPERATIONS},
      author = {Ben Nimmo},
      url    = {https://www.brookings.edu/wp-content/uploads/2020/09/Nimmo_influence_operations_PDF.pdf},
      year   = {2021 (accessed January 5, 2021}
}
% following are publications from Harvard Misinformation Review
@manual{tackling-misinformation,
      title  = {Tackling misinformation: What researchers could do with social media data},
      author = {Pasquetto, Irene V. and Swire-Thompson, Briony and Amazeen, Michelle A. and others},
      publisher= {The Harvard Kennedy School (HKS) Misinformation Review},
      url = {https://doi.org/10.37016/mr-2020-49},
      year   = {2021 (accessed January 8, 2021}
}
@manual{misinformation-4chan-Reddit,
      title  = {Research note: The spread of political misinformation on online subcultural platforms},
      author = {BURTON, ANTHONY G. and KOEHORS, DIMITRI},
      publisher= {The Harvard Kennedy School (HKS) Misinformation Review},
      url = {https://doi.org/10.37016/mr-2020-40},
      year   = {2021 (accessed January 13, 2021}
}
@manual{cross-platform-white-helmets,
      title  = {Cross-platform disinformation campaigns: lessons learned and next steps},
      author = {Wilson, Tom and Starbird, Kate},
      publisher= {The Harvard Kennedy School (HKS) Misinformation Review},
      url = {https://doi.org/10.37016/mr-2020-002},
      year   = {2021 (accessed January 13, 2021}
}
@manual{cross-platform-covid19-conspiracy,
      title  = {The spread of COVID-19 conspiracy theories on social media and the effect of content moderation},
      author = {PAPAKYRIAKOPOULOS, ORESTIS and SERRANO, JUAN CARLOS MEDINA and HEGELICH, SIMON},
      publisher= {The Harvard Kennedy School (HKS) Misinformation Review},
      url = {https://doi.org/10.37016/mr-2020-034},
      year = {2021 (accessed January 13, 2021}
}
@manual{twitter-origin-evolution-covid19-plandemic,
      title  = {The Twitter origins and evolution of the COVID-19 "plandemic" conspiracy theory},
      author = {KEARNEY, MATTHEW D. and CHIANG, SHAWN C. and MASSEY, PHILIP M.},
      publisher= {The Harvard Kennedy School (HKS) Misinformation Review},
      url = {https://doi.org/10.37016/mr-2020-42},
      year = {2021 (accessed January 13, 2021}
}
@inproceedings{known-unknown,
author = {Tanash, Rima S. and Chen, Zhouhan and Thakur, Tanmay and Wallach, Dan S. and Subramanian, Devika},
title = {Known Unknowns: An Analysis of Twitter Censorship in Turkey},
year = {2015},
isbn = {9781450338202},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2808138.2808147},
doi = {10.1145/2808138.2808147},
booktitle = {Proceedings of the 14th ACM Workshop on Privacy in the Electronic Society},
pages = {11–20},
numpages = {10},
keywords = {twitter, social networks, censorship},
location = {Denver, Colorado, USA},
series = {WPES '15}
}
@article {spread-of-true-and-false-news,
	author = {Vosoughi, Soroush and Roy, Deb and Aral, Sinan},
	title = {The spread of true and false news online},
	volume = {359},
	number = {6380},
	pages = {1146--1151},
	year = {2018},
	doi = {10.1126/science.aap9559},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {https://science.sciencemag.org/content/359/6380/1146},
	eprint = {https://science.sciencemag.org/content/359/6380/1146.full.pdf},
	journal = {Science}
}

@article{application-fake-news-in-health,
	An = {32260048},
	Author = {Pulido, Cristina M and Ruiz-Eugenio, Laura and Redondo-Sama, Gisela and Villarejo-Carballido, Beatriz},
	Date = {2020/04/03},
	Date-Added = {2021-01-08 19:14:43 +0000},
	Date-Modified = {2021-01-08 19:14:43 +0000},
	Db = {PubMed},
	Doi = {10.3390/ijerph17072430},
	Isbn = {1660-4601; 1661-7827},
	J2 = {Int J Environ Res Public Health},
	Journal = {International journal of environmental research and public health},
	Keywords = {*Ebola; *fake news; *nutrition; *public health; *social impact in social media; *social media analysis; *vaccines; *Deception; Health; Mass Media; Social Change; *Social Media; *Trust},
	L2 = {https://www.ncbi.nlm.nih.gov/pmc/articles/PMC7177765/},
	La = {eng},
	Month = {04},
	Number = {7},
	Pages = {2430},
	Publisher = {MDPI},
	Title = {A New Application of Social Impact in Social Media for Overcoming Fake News in Health},
	Ty = {JOUR},
	U1 = {32260048{$[$}pmid{$]$}},
	U2 = {PMC7177765{$[$}pmcid{$]$}},
	U4 = {ijerph17072430{$[$}PII{$]$}},
	Url = {https://pubmed.ncbi.nlm.nih.gov/32260048},
	Volume = {17},
	Year = {2020},
	Bdsk-Url-1 = {https://pubmed.ncbi.nlm.nih.gov/32260048},
	Bdsk-Url-2 = {http://dx.doi.org/10.3390/ijerph17072430}
}
@article{internet-user-engage-facebook,
	Author = {Berriche, Manon and Altay, Sacha},
	Da = {2020/04/28},
	Date-Added = {2021-01-08 19:20:43 +0000},
	Date-Modified = {2021-01-08 19:20:43 +0000},
	Doi = {10.1057/s41599-020-0452-1},
	Id = {Berriche2020},
	Isbn = {2055-1045},
	Journal = {Palgrave Communications},
	Number = {1},
	Pages = {71},
	Title = {Internet users engage more with phatic posts than with health misinformation on Facebook},
	Ty = {JOUR},
	Url = {https://doi.org/10.1057/s41599-020-0452-1},
	Volume = {6},
	Year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1057/s41599-020-0452-1},
	Bdsk-Url-2 = {http://dx.doi.org/10.1057/s41599-020-0452-1}
}
@manual{statista-social-networking-apps-rank,
      title  = {Most popular mobile social networking apps in the United States as of September 2019},
      author = {Statista},
      url = {https://www.statista.com/statistics/248074/most-popular-us-social-networking-apps-ranked-by-audience/},
      year   = {2020 (accessed January 8, 2021)}
}
@article {less-than-you-think,
	author = {Guess, Andrew and Nagler, Jonathan and Tucker, Joshua},
	title = {Less than you think: Prevalence and predictors of fake news dissemination on Facebook},
	volume = {5},
	number = {1},
	elocation-id = {eaau4586},
	year = {2019},
	doi = {10.1126/sciadv.aau4586},
	publisher = {American Association for the Advancement of Science},
	URL = {https://advances.sciencemag.org/content/5/1/eaau4586},
	eprint = {https://advances.sciencemag.org/content/5/1/eaau4586.full.pdf},
	journal = {Science Advances}
}
@inproceedings{proactive-discovery-of-fake-news,
author = {Chen, Zhouhan and Freire, Juliana},
title = {Proactive Discovery of Fake News Domains from Real-Time Social Media Feeds},
year = {2020},
isbn = {9781450370240},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3366424.3385772},
doi = {10.1145/3366424.3385772},
booktitle = {Companion Proceedings of the Web Conference 2020},
pages = {584–592},
numpages = {9},
keywords = {misinformation, social network analysis, fake news discovery},
location = {Taipei, Taiwan},
series = {WWW '20}
}
@article{Fake-News-and-Covid-19-in-Italy,
	An = {32806772},
	Author = {Moscadelli, Andrea and Albora, Giuseppe and Biamonte, Massimiliano Alberto and Giorgetti, Duccio and Innocenzio, Michele and Paoli, Sonia and Lorini, Chiara and Bonanni, Paolo and Bonaccorsi, Guglielmo},
	Date = {2020/08/12},
	Date-Added = {2021-01-08 20:02:41 +0000},
	Date-Modified = {2021-01-08 20:02:41 +0000},
	Db = {PubMed},
	Doi = {10.3390/ijerph17165850},
	Isbn = {1660-4601; 1661-7827},
	J2 = {Int J Environ Res Public Health},
	Journal = {International journal of environmental research and public health},
	Keywords = {*BuzzSumo; *Covid-19; *coronavirus; *fake news; *health literacy; *social media; Betacoronavirus; COVID-19; Communications Media/*standards/*statistics \& numerical data; Coronavirus Infections/*epidemiology; Health Communication/*standards; Health Literacy; Humans; Italy/epidemiology; Pandemics; Pneumonia, Viral/*epidemiology; SARS-CoV-2},
	L2 = {https://www.ncbi.nlm.nih.gov/pmc/articles/PMC7459609/},
	La = {eng},
	Month = {08},
	Number = {16},
	Pages = {5850},
	Publisher = {MDPI},
	Title = {Fake News and Covid-19 in Italy: Results of a Quantitative Observational Study},
	Ty = {JOUR},
	U1 = {32806772{$[$}pmid{$]$}},
	U2 = {PMC7459609{$[$}pmcid{$]$}},
	U4 = {ijerph17165850{$[$}PII{$]$}},
	Url = {https://pubmed.ncbi.nlm.nih.gov/32806772},
	Volume = {17},
	Year = {2020},
	Bdsk-Url-1 = {https://pubmed.ncbi.nlm.nih.gov/32806772},
	Bdsk-Url-2 = {http://dx.doi.org/10.3390/ijerph17165850}
}
@misc{tools-fight-misinformation,
  author = {The RAND Corporation},
  title = {{Tools That Fight Disinformation Online
}},
  howpublished = {\url{https://www.rand.org/research/projects/truth-decay/fighting-disinformation/search.html}},
  year = {2019}, 
  note = "[Online; accessed 13-January-2021]"
}
@misc{covid19-misinformation-twitter-dashboard,
      title={COVID-19 on Social Media: Analyzing Misinformation in Twitter Conversations}, 
      author={Karishma Sharma and Sungyong Seo and Chuizheng Meng and Sirisha Rambhatla and Yan Liu},
      year={2020},
      eprint={2003.12309},
      archivePrefix={arXiv},
      primaryClass={cs.SI}
}
@inproceedings{known-unknown-twitter-censorship,
author = {Tanash, Rima S. and Chen, Zhouhan and Thakur, Tanmay and Wallach, Dan S. and Subramanian, Devika},
title = {Known Unknowns: An Analysis of Twitter Censorship in Turkey},
year = {2015},
isbn = {9781450338202},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2808138.2808147},
doi = {10.1145/2808138.2808147},
booktitle = {Proceedings of the 14th ACM Workshop on Privacy in the Electronic Society},
pages = {11–20},
numpages = {10},
keywords = {social networks, twitter, censorship},
location = {Denver, Colorado, USA},
series = {WPES '15}
}
@misc{conservative-site-ranking,
  author = {Paula Bolyard},
  title = {{Top 50 Conservative Websites for 2018}},
  howpublished = "\url{https://www.math.uwaterloo.ca/~hwolkowi//house.d/Top50ConservativeWebsitesfor2018.htm}",
  year = {2018}, 
  note = "[Online; accessed 3-February-2021]"
}
@misc{yang-covid19-infodemic,
      title={The COVID-19 Infodemic: Twitter versus Facebook}, 
      author={Kai-Cheng Yang and Francesco Pierri and Pik-Mai Hui and David Axelrod and Christopher Torres-Lugo and John Bryden and Filippo Menczer},
      year={2020},
      eprint={2012.09353},
      archivePrefix={arXiv},
      primaryClass={cs.SI}
}
@misc{pierri-2021-vaccinitaly,
      title={VaccinItaly: monitoring Italian conversations around vaccines on Twitter}, 
      author={Francesco Pierri and Silvio Pavanetto and Marco Brambilla and Stefano Ceri},
      year={2021},
      eprint={2101.03757},
      archivePrefix={arXiv},
      primaryClass={cs.SI}
}
@article{twitter-user-aggregate-characterization,
author = {Bild, David R. and Liu, Yue and Dick, Robert P. and Mao, Z. Morley and Wallach, Dan S.},
title = {Aggregate Characterization of User Behavior in Twitter and Analysis of the Retweet Graph},
year = {2015},
issue_date = {February 2015},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {15},
number = {1},
issn = {1533-5399},
url = {https://doi.org/10.1145/2700060},
doi = {10.1145/2700060},
journal = {ACM Trans. Internet Technol.},
month = mar,
articleno = {4},
numpages = {24},
keywords = {decentralized network architectures, microblogging systems, Social network analysis}
}
@article{lancet-infodemic,
	Annote = {doi: 10.1016/S0140-6736(20)30461-X},
	Author = {Zarocostas, John},
	Booktitle = {The Lancet},
	Date = {2020/02/29},
	Date-Added = {2021-02-19 19:28:33 +0000},
	Date-Modified = {2021-02-19 19:28:33 +0000},
	Doi = {10.1016/S0140-6736(20)30461-X},
	Isbn = {0140-6736},
	Journal = {The Lancet},
	M3 = {doi: 10.1016/S0140-6736(20)30461-X},
	Month = {2021/02/19},
	Number = {10225},
	Pages = {676},
	Publisher = {Elsevier},
	Title = {How to fight an infodemic},
	Ty = {JOUR},
	Url = {https://doi.org/10.1016/S0140-6736(20)30461-X},
	Volume = {395},
	Year = {2020},
	Year1 = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0140-6736(20)30461-X},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/S0140-6736(20)30461-X}
}
@misc{doubleverify-report,
  title = {{Global Online Content Consumption Doubles in 2020}},
  howpublished = "\url{https://doubleverify.com/newsroom/global-online-content-consumption-doubles-in-2020-research-shows/}",
  year = {2020}, 
  note = "[Online; accessed 22-February-2021]"
}
@misc{nielsen-report,
  title = {{COVID-19: TRACKING THE IMPACT ON MEDIA CONSUMPTION}},
  howpublished = "\url{https://www.nielsen.com/us/en/insights/article/2020/covid-19-tracking-the-impact-on-media-consumption/}",
  year = {2020}, 
  note = "[Online; accessed 22-February-2021]"
}
@misc{mozilla-referrer,
  title = {{Referrers by default to protect user privacy}},
  howpublished = "\url{https://blog.mozilla.org/security/2021/03/22/firefox-87-trims-http-referrers-by-default-to-protect-user-privacy/}",
  year = {2021}, 
  note = "[Online; accessed 24-June-2021]"
}
@manual{misinformation-in-action,
      title  = {Misinformation in action: Fake news exposure is linked to lower trust in media, higher trust in government when your side is in power},
      author = {OGNYANOVA, KATHERINE and LAZER, DAVID and ROBERTSON, RONALD E. and WILSON, CHRISTO},
      publisher= {The Harvard Kennedy School (HKS) Misinformation Review},
      url = {https://doi.org/10.37016/mr-2020-024},
      year   = {2020}
}

